Towards Principled, Practical Policy Gradient for Bandits and Tabular MDPs

We consider (stochastic) softmax policy gradient (PG) methods for bandits and tabular Markov decision processes (MDPs). While the PG objective is non-concave, recent research has used the objective's smoothness and gradient domination properties to achieve convergence to an optimal policy. However, these theoretical results require setting the algorithm parameters according to unknown problem-dependent quantities (e.g. the optimal action or the true reward vector in a bandit problem). To address this issue, we borrow ideas from the optimization literature to design practical, principled PG methods in both the exact and stochastic settings. In the exact setting, we employ an Armijo line-search to set the step-size for softmax PG and demonstrate a linear convergence rate. In the stochastic setting, we utilize exponentially decreasing step-sizes, and characterize the convergence rate of the resulting algorithm. We show that the proposed algorithm offers similar theoretical guarantees as the state-of-the art results, but does not require the knowledge of oracle-like quantities. For the multi-armed bandit setting, our techniques result in a theoretically-principled PG algorithm that does not require explicit exploration, the knowledge of the reward gap, the reward distributions, or the noise. Finally, we empirically compare the proposed methods to PG approaches that require oracle knowledge, and demonstrate competitive performance.

==> 4_pg_with_entropy.tex <==
\section{Policy Gradient With Entropy Regularization in the Exact Setting}\label{section:pg_w_entropy}
\red{Why entropy}

Let $\ftau(\theta)= f(\theta) + \tau \, \sH(\pitheta)$ denote the entropy regularized objective where $\tau \geq 0$ is the strength of the denotes the strength of the entropy regularization and $\fstartau := \max_{\theta} \ftau(\theta)$ denote the optimal entropy regularized objective. For a given $\tau$, $\ftau$ is $L^\tau$ uniform-smooth and 
furthermore, $\ftau$ now satisfies non-uniform \L ojasiewciz condition with $C_\tau(\theta)$ and $\xi = \nicefrac{1}{2}$. \cref{table:entropy} summarizes the entropy regularizer, uniform smoothness and non-uniform \L ojsaiewciz properties for bandits and general MDPs with entropy regularization.
In the subsequent sections, we assume that $\mu := \inf_{t \geq 1}  C_\tau^2(\thetat) > 0$ and $\tau \in [0, 1]$.

\red{Define $\mu$ only in the theorem.}

\begin{table}[h]\small
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Setting&  
$\mathbb{H}(\pitheta)$&
$L$&
$C_\tau(\theta)$
\\ \hline
\begin{tabular}[c]{@{}c@{}}Bandits with \\  Entropy Regularization\end{tabular}&
$- \log \pitheta$&
$5/2 + 5\tau(1 +  \log \abs{\gA})$&
$\sqrt{2 \tau} \min_a \pitheta(a)$ 
\\\hline
\begin{tabular}[c]{@{}c@{}}Tabular MDP with \\  Entropy Regularization\end{tabular}&
$\E \bracks*{\sum_{t=0}^\infty -\gamma^t \log \pitheta(a_t | s_t)}$& 
$\frac{8 + \tau(4 + 8 \log \abs{\gA})}{(1 - \gamma)^3}$ &
$\frac{\sqrt{\tau} \min_s \sqrt{\rho(s)} \, \min_{s, a} \pitheta(a |s)}{\abs{\gS}\supnorm{d^{\pi^{*_\tau}}_\rho / d^{\pitheta}_\rho}^{1/2} }$
\\ \hline
\end{tabular}
\caption{Entropy Regularizer, uniform smoothness and non-uniform \L ojasiewciz condition with $\xi = \nicefrac{1}{2}$ for bandit and general tabular MDPs with entropy regularization. 
}
\label{table:entropy}
\end{table}


The update for the entropy regularized objective is given as,
\begin{update}(Softmax PG with Entropy Regularization, True Gradient)\label{update:entropy_pg}
\\ \indent\indent\indent$\theta_{t+1} = \theta_t + \nabla \ftau(\thetat)$ 
\end{update}

\red{SPG + Entropy - only with constant step-size}

\red{Jincheng gets 1/T rate to a biased policy. Recalling}

The resulting policy is biased due to the presence of entropy regularization. 
In order for entropy regularized objectives to converge to the globally optimal policy, $\tau \rightarrow 0$.
Using \cref{update:entropy_pg}, prior work~\citep{mei2020global} used a two-stage approach to decay $\tau$, but the resulting algorithm requires knowledge of $\Delta$, rendering the method ineffective.

\red{Multi-stage algorithm to get convergence without knowledge of $\Delta$ or other problem-dependent parameters}

\red{Abstract out Algorithm 2/3 in the Appendix and put it here: similar to https://arxiv.org/pdf/2302.02607.pdf}

\red{Add Theorem from Appendix D -- $B_1$, $B_2$ assumptions}

\red{Corollary: Bandits. Require knowledge of $\mu_i$ for every stage $i$. Unfortunately, do not know this and approximate it (use Matin's explanation) and set it to $\tau^2$ (cite the result in the Appendix that shows that true $\mu$ is close to the estimated $\mu$. )}.

\red{Put the experiment result}

We note that in the proof we treat $c := \inf_{t \geq 0} \min_a \pi_{\theta_t}(a)$ and hence $\mu$ as a constant. We conjecture that there is a hidden strong dependence on $\eps$ in $c$, and that this dependence can be weakened by proving a tighter bound on $\mu$.
Unfortunately, using a fixed $\tau$ leads to a $\gO\left(\nicefrac{1}{\epsilon} \log{\nicefrac{1}{\epsilon}}\right)$ convergence rate that is slower than PG methods without the presence of entropy. 
Thus, we present~\cref{algorithm:multi_stage} that decays the entropy in stages and achieves a $\gO\left(\nicefrac{1}{\eps}\right)$ rate, matching the two-stage approach in~\citep{mei2020global}, but without requiring the prior knowledge of $\Delta$. Additionally, in comparison to~\cref{theorem:fixed_tau}, the algorithm do not require $\eps$ to be set in advance. We analyze ~\cref{algorithm:multi_stage} and prove its convergence rate in \cref{appendix:proof_multi_stage}. 


==> 5_spg_with_entropy.tex <==
 \section{Stochastic Policy Gradient With Entropy Regularization}\label{section:spg_w_entropy}
Following \cref{section:spg_wo_entropy}, we construct a gradient estimator using IS for the entropy regularized objective. This estimator $\htgrad{\thetat}$ has been shown to be unbiased and has bounded variance~\citep{ding2023local}, i.e. $\E \normsq{\htgrad{\thetat} - \E[\htgrad{\thetat}]} \leq b := 8 (1 + (\tau \, \log{|\gA|})^2)$. We consider the following update,
\begin{update}(Stochastic Softmax PG  with Entropy, Importance Sampling)\label{update:entropy_spg}
\\ \indent\indent\indent$\theta_{t+1} = \theta_t + \htgrad{\thetat} = \thetat + \etat H(\pitheta)(\hat{r} - \tau \log \pitheta)$
\end{update}
Under the same setting, prior work~\citep{ding2021beyond} proposes a two-stage approach that converges to a globally optimal policy by modifying the batch size to counteract the variance at a $\tilde{\gO}(\nicefrac{1}{\eps^2})$ convergence rate, but requires knowledge of the optimal policy to set the algorithm parameters. Using the same rationale as in~\cref{section:spg_wo_entropy}, using ~\cref{update:entropy_spg} with fixed $\tau$ and in conjunction with an exponentially decaying step-size to mitigate the variance, we can converge to an $\eps$-neighbourhood of a globally optimal policy after $\tilde{\gO}\left(\nicefrac{1}{\epsilon} + \nicefrac{b}{\epsilon^3}\right)$ iterations. We prove the following theorem in~\cref{appendix:proof_sto_fixed_tau}. 
\begin{restatable}{theorem}{theoremStoFixedTau}\label{theorem:sto_fixed_tau}
Assuming $c := \inf_{t \geq 0} \min_a \pi_{\theta_t}(a) > 0$, using~\cref{update:entropy_spg} with $\tau = \epsilon / \left(2 \left(W\left(\nicefrac{|\gA| - 1}{e}\right) + \log{|\gA|}\right)\right)$ and using exponential decreasing step-size $\eta_t = \nicefrac{\alpha^{t + 1}}{L^\tau}$,
achieves
$\epsilon$-suboptimality after $\tilde{\gO}\left(\nicefrac{1}{\epsilon} + \nicefrac{b}{\epsilon^3}\right)$ iterations. 
\end{restatable}
Finally, we extend the multi-stage approach of~\cref{algorithm:multi_stage} to the stochastic setting, resulting in~\cref{algorithm:sto_multi_stage} in~\cref{appendix:proof_sto_multi_stage}. In~\cref{theorem:sto_multi_stage} in~\cref{appendix:proof_sto_multi_stage}, we prove an $\tilde{\gO}\left(\nicefrac{1}{\epsilon} + \nicefrac{b}{\epsilon^3}\right)$ convergence rate for the resulting algorithm. 
This matches the corresponding rate in~\cref{theorem:spg_ess}. 


==> header.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amscd}
\usepackage{amsfonts}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{wrapfig}
\usepackage{subcaption}
\PassOptionsToPackage{algo2e,ruled}{algorithm2e}
\RequirePackage{algorithm2e}
\setlength\algomargin{0pt}
% \usepackage{algorithmic}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{amssymb,amsmath}
% \usepackage{amsthm}

\usepackage{thmtools, thm-restate}
\usepackage[mathscr]{eucal} % for mathscr
\usepackage[round]{natbib}
\usepackage{bbm}
\usepackage{bm}
\usepackage{arydshln}
\usepackage{enumitem}
\usepackage{cancel}
\usepackage{graphicx}
\usepackage{mdframed}
\usepackage{pgfplots}
\usepackage[normalem]{ulem}
\usepackage{mathtools}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{xargs}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{adjustbox}
\usepackage{soul}
\usepackage{float}
% \usepackage{tabularx}
% \usepackage{multirow}
% \usepackage{makecell}


\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\ml}[1]{\textcolor{blue}{ml: #1}}

\newcommand{\unsure}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{#1}}

\newcommand{\mlunsure}[1]{\todo[inline, linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{#1}}

\newcommand{\unsureil}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue, inline]{#1}}



% \newcommand{\val}[1]{\textcolor{ForestGreen}{#1}}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\usepackage[colorlinks=true,
    linkcolor=mydarkblue,
    citecolor=mydarkblue,
    filecolor=mydarkblue,
    urlcolor=mydarkblue,
    pagebackref=true]{hyperref} 
\usepackage[capitalize, noabbrev]{cleveref}
\renewcommand*\backref[1]{\ifx#1\relax \else (cited on #1) \fi}

\definecolor{shadecolor}{gray}{0.90}
\declaretheoremstyle[
headfont=\normalfont\bfseries,
notefont=\mdseries, notebraces={(}{)},
bodyfont=\normalfont,
postheadspace=0.5em,
spaceabove=5pt,
mdframed={
  skipabove=3pt,
  skipbelow=3pt,
  hidealllines=true,
  backgroundcolor={shadecolor},
  innerleftmargin=2pt,
  innerrightmargin=2pt}
]{shaded}

\declaretheorem[style=shaded]{theorem}
\declaretheorem[style=shaded]{corollary}
% \newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{defn}{Definition}
\newtheorem{update}{Update}
\newtheorem{assumption}{Assumption}
\crefname{assumption}{assumption}{assumptions}

\mdfdefinestyle{mdframedthmbox}{%
	leftmargin=.0\textwidth,
	rightmargin=.0\textwidth,%
	innertopmargin=0.75em,
	innerleftmargin=.5em,
	innerrightmargin=.5em,
}

\newenvironment{thmbox}
	{%
		\begin{mdframed}[style=mdframedthmbox]%
	}{% 
		\end{mdframed}%
	}
\newcommand{\myquote}[1]{\null~\\{\null\hspace{.05\textwidth}\begin{minipage}[t]{.90\textwidth} #1 \end{minipage}}}
\newcommand{\myquoten}[1]{{\null\hspace{.05\textwidth}\begin{minipage}[t]{.90\textwidth} #1 \end{minipage}}}

\setlength{\intextsep}{1\baselineskip}

\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}

\makeatletter
\def\thm@space@setup{\thm@preskip=0pt
\thm@postskip=0pt}
\makeatother

